On Groups $G_{n}^{k}$ and $\Gamma_{n}^{k}$: A Study of Manifolds, Dynamics, and Invariants

Recently the first named author defined a 2-parametric family of groups $G_n^k$. Those groups may be regarded as analogues of braid groups. Study of the connection between the groups $G_n^k$ and dynamical systems led to the discovery of the following fundamental principle: If dynamical systems describing the motion of $n$ particles possess a nice codimension 1 property governed by exactly $k$ particles, then these dynamical systems admit a topological invariant valued in $G_{n}^{k}$. The $G_n^k$ groups have connections to different algebraic structures. Study of the $G_n^k$ groups led to, in particular, the construction of invariants, valued in free products of cyclic groups. All generators of the $G_{n}^{k}$ groups are reflections but there are many ways to enhance them to get rid of $2$-torsion. Later the first and the fourth named authors introduced and studied the second family of groups, denoted by $\Gamma_n^k$, which are closely related to triangulations of manifolds. The spaces of triangulations of a given manifolds have been widely studied. Theorem of Pachner says that any two triangulations of a given manifold can be connected by a sequence of bistellar moves or Pachner moves. $\Gamma_n^k$ naturally appear when considering the set of triangulations with the fixed number of points. There are two ways of introducing $\Gamma_n^k$: the geometrical one, which depends on the metric, and the topological one. The second one can be thought of as a {\guillemotleft}braid group{\guillemotright} of the manifold and is an invariant of the topological type of manifold; in a similar way, one can construct the smooth version. In the present paper we give a survey of the ideas lying in the foundation of the $G_n^k$ and $\Gamma_n^k$ theories and give an overview of recent results in the study of those groups, manifolds, dynamical systems, knot and braid theories.

==> abstract_old.tex <==
Recently the first named author defined a 2-parametric family of groups $G_n^k$ \cite{gnk}. Those groups may be regarded as a certain generalisation of braid groups. Study of the connection between the groups $G_n^k$ and dynamical systems led to the discovery of the following fundamental principle: ``If dynamical systems describing the motion of $n$ particles possess a nice codimension one property governed by exactly $k$ particles, then these dynamical systems admit a topological invariant valued in $G_{n}^{k}$''.

The $G_n^k$ groups have connections to different algebraic structures, Coxeter groups and Kirillov-Fomin algebras, to name just a few. Study of the $G_n^k$ groups led to, in particular, the construction of invariants, valued in free products of cyclic groups.

Later the first and the fourth named authors introduced and studied the second family of groups, denoted by $\Gamma_n^k$, which are closely related to triangulations of manifolds.

The spaces of triangulations of a given manifolds have been widely studied. The celebrated theorem of Pachner~\cite{pach} says that any two triangulations of a given manifold can be connected by a sequence of bistellar moves or Pachner moves. See also~\cite{GelKapZel,nab}; the $\Gamma_n^k$ naturally appear when considering the set of triangulations with the fixed number of points.

There are two ways of introducing the groups $\Gamma_n^k$: the geometrical one, which depends on the metric, and the topological one. The second one can be thought of as a ``braid group'' of the manifold and, by definition, is an invariant of the topological type of manifold; in a similar way, one can construct the smooth version.

In the present paper we give a survey of the ideas lying in the foundation of the $G_n^k$ and $\Gamma_n^k$ theories and give an overview of recent results in the study of those groups, manifolds, dynamical systems, knot and braid theories. 

==> decorated_triangulation.tex <==
\section{A representation of braids via decorated triangulations}
The purpose of the present section is to introduce the notion of decorated triangulation and to construct a representation of braids group. 

\begin{definition}
{\em A decorated triangulation} is a triangulation where all triangles are linearly ordered and in each triangle, a distinguished corner is fixed.
\end{definition}

An example of a decorated triangulation of the disk with 5 points is described in Fig.~\ref{exa_decorated_triang}.
\begin{figure}
\centering\includegraphics[width=100pt]{pics/exa_decorated_triang.eps}
\caption{A decorated ideal triangulation of the disk}
\label{exa_decorated_triang}
\end{figure}


\begin{definition}\label{def:BAS}
Let $\mathcal{C} = (\mathcal{C}, \otimes, \{P_{X,Y}\}_{X,Y \in Ob\mathcal{C}})$ be a symmetric monoidal category. A {\em basic algebraic system} (BAS) in $\mathcal{C}$ consists of an object $V \in Ob\mathcal{C}$ and two morphisms $R \in End(V)$ and $W \in End(V\otimes V)$ such that
\begin{enumerate}
\item $R_{i}^{3} = id_{V}$,
\item $W_{i,j}W_{j,k} = W_{j,k}W_{i,k}W_{i,j}$ in $End(V^{\otimes 3})$,
\item $R_{i}R_{j}W_{j,i}R_{i}^{-1}W_{i,j} = P_{i,j}$ in $End(V^{\otimes 2})$, where $P_{i,j} :=P_{V,V}$.
\end{enumerate}

\end{definition}

The morphisms $R_{i} : V \rightarrow V$ and $W_{i,j} : V \otimes V \rightarrow V \otimes V$ correspond to distinguished corner changes and the flip, respectively, see Fig.~\ref{corner_flip}.

\begin{figure}
\centering\includegraphics[width=150pt]{pics/corner_flip.eps}
\caption{Distinguished corner changes and the flip}
\label{corner_flip}
\end{figure}

Moreover the conditions (2) and (3) from Definition~\ref{def:BAS} can be described by the pentagon relation and changes of the order of triangles, see Fig.~\ref{pentagon_BAS} and Fig.~\ref{geo_change_order_BAS}.
\begin{figure}
\centering\includegraphics[width=250pt]{pics/pentagon_BAS.eps}
\caption{Geometric description of the condition (2) from Definition~\ref{def:BAS}}
\label{pentagon_BAS}
\end{figure}

\begin{figure}
\centering\includegraphics[width=200pt]{pics/geo_change_order_BAS.eps}
\caption{Geometric description of the condition (3) from Definition~\ref{def:BAS}}
\label{geo_change_order_BAS}
\end{figure}

\begin{example}\label{exa:BAS_Ptolemy}
Let ${\bf Set}$ be the category of sets with monoidal structure given by the cartesian product, and the transpositions of the components. Let $V = \mathbb{R}_{+}^{2}$ and define $R : V \rightarrow V$ and $W : V \times V \rightarrow V \times V$ by

\begin{equation}
R(x_{1},x_{2}) = (\frac{1}{x_{1}},\frac{x_{2}}{x_{1}}), W((x_{1},x_{2}),(y_{1},y_{2})) = (\frac{x_{2}y_{1}}{x_{1}y_{2}+x_{2}}, \frac{y_{2}}{x_{1}y_{2}+x_{2}}).
\end{equation}
Then this is a BAS.
\end{example}

Let us consider the set of all ordered triangulation of $\Sigma$ with $N$ enumerated vertices as the previous section. For each triangulation $\tau$ of $\Sigma$ we can obtain a decorated triangulation $\tilde{\tau}$ by fixing a corner for each triangle. Recall that in the previous section edges of $\tau$ are considered as variables. Now we define a map from triangles of $\tilde{\tau}$ to $\mathbb{Q}(x_{1}, \cdots, x_{X}) \times \mathbb{Q}(x_{1}, \cdots, x_{X})$ as described in Fig.~\ref{ratio_coordinate}.

\begin{figure}
\centering\includegraphics[width=150pt]{pics/ratio_coordinate.eps}
\caption{$a,b,c \in \mathbb{Q}(x_{1}, \cdots x_{X})$, which are associated to each edge of the triangulation $\tau$}
\label{ratio_coordinate}
\end{figure}



==> introduction_old.tex <==
A long time ago, when I first encountered knot tables and started unknotting knots ``by hand'', I was quite excited with the fact that some knots may have more than one minimal representative. In other words, in order to make an object simpler, one should first make it more complicated, for example, see Fig.~\ref{culprit_knot} \cite{KauffmanLambropoulou}: this diagram represents the trivial knot, but in order to simplify it, one needs to perform an {\em increasing} Reidemeister move first.

\begin{figure}[t!]
\begin{center}
 \includegraphics[width = 4cm]{pics/culprit_knot.eps}

\end{center}

\caption{Culprit knot}\label{culprit_knot}
\end{figure}

Being a first year undergraduate student (in the Moscow State University), I first met free groups and their presentation. The power and beauty, and simplicity of these groups for me were their exponential growth and extremely easy solution to the word problem and conjugacy problem by means of a gradient descent algorithm in a word (in a cyclic word, respectively).

Also, I was excited with Diamond lemma (see Fig. \ref{diamond}): a simple condition which guarantees the uniqueness of the minimal objects, and hence, solution to many problems.

Being a last year undergraduate and teaching a knot theory course for the first time,  I thought: ``Why do not we have it (at least partially) in knot theory?''

%%%%%%%%%%%%%%%%Zieschang...

By that time I knew about the Diamond lemma and solvability of many problems like word problem in groups by gradient descent algorithm. The van Kampen lemma and the Greendlinger theorem came to my knowledge much later.

\begin{figure}[t!]
\begin{center}
 \includegraphics[width = 40mm]{pics/simple_diamond.eps}
\end{center}
\caption{The Diamond lemma}\label{diamond}
\end{figure}


Virtual knot theory \cite{Kauffman_virtual_knots, Kam, abstract, GPV}, which can be formally defined via Gau{\ss} diagrams which are not necessarily planar, is a theory about knots in thickened surfaces $S_{g}\times I$ considered up to addition/removal of nugatory handles. It contains classical knot theory as a proper part: classical knots can be thought of as knots in the thickened sphere. Hence, virtual knots have a lot of additional information coming from the topology of the ambient space ($S_{g})$.

By playing with formal Gau{\ss} diagrams, I decided to drop any arrow and sign information and called such objects {\em free knots}~\cite{ManFreeKnot}.


In January, 2009, I constructed a state-sum invariant of free knots valued in diagrams of free knots, i.e., framed four-valent graphs\footnote{After I constructed such invariant, I learnt that free knots were invented by Turaev five years before that and thought to be trivial \cite{tur}, hence, I disproved Turaev's conjecture without knowing that.} \cite{knot_parity}. For states, I was taking all possible smoothings at even (in some sense) crossings, imposing some diagrams to be zero. This invariant was constructed in such a way that all odd chord persisted and I got the formula~$$[K]=K$$ whenever $K$ is a diagram of a free knot with all chords odd where no two chords can be cancelled by a second Reidemeister move.

The deep sense of this formula can be expressed as follows: \\

{\em If a virtual diagram is complicated enough, then it realises itself.} \\

Namely, $K$ on the left hand side is {\em some} free knot diagram $K$, i.e. an equivalence class, and $K$ on the right hand side is a {\em concrete graph}. Hence, if $K'$ is another diagram of the same knot, we shall have $[K']=K$ meaning that $K$ is obtained as a result of smoothing of $K'$. This principle is depicted on Fig. \ref{cat}.

\begin{figure}
\centering\includegraphics[width=200pt]{pics/catrus.eps}
\caption{A picture which is its own invariant}
\label{cat}
\end{figure}

This is an example of what we miss in classical knot theory: {\em local minimality yields global minimality} or, in other words, {\em if a diagram is odd and irreducible} then it is {\em minimal} in a very strong sense. Not only one can say that $K'$ has larger crossing number than $K$, we can say that $K$ ``lives'' inside $K'$. Having these ``graphical'' invariants, we get immediate consequences about many characteristics of $K$. \\ %The main problem is to construct invariants of similar nature for classical knots. \\

Something similar we see in other situations: free groups or free products of cyclic groups, cobordism theory for free knots, or while considering other geometrical problems. For example, if we want to understand the genus of a surface where the knot $K$ can be realised, it suffices for us to look at the minimal genus where the concrete diagram $K$ can be realised, for the genus of any other $K'$ is a priori larger than that of $K$ \cite{Manturov_virtual_number}, see also \cite{IMN1}.

The diagrammatic approach takes me back to the time of my habilitation thesis. Once writing a knot theory paper and discussing it with Oleg Yanovich Viro, I wrote ``a classical knot is an equivalence class of classical knot diagrams modulo Reidemeister moves''. ``Well, --- said Viro, --- you are restricting yourself very much. Staying at this position, how can you prove that a non-trivial knot has a quadrisecant?''

Reflecting this after several years and having published several knot theory books \cite{M_knot_theory, Book, IMN1}, I understood that it is not quite necessary to  consider knots by using Reidemeister planar projections, one can look for other ``nodes''.

This led me to my initial preprint~\cite{gnk} %%%Non-Reidemeister knot theory
and to an extensive study of braids and dynamical systems. This happened around New Year 2015.

Namely, I looked at usual Artin's braids as everybody does: as dynamical systems of points in $\R^{2}$, but, instead of creating Reidemeister's diagram by projecting braids to a screen (say, the plane $Oxz$), I decided to look at those moments when some three points are {\em collinear}. This is quite a good property of a ``node'' which behaves nicely under generic isotopy. Let us denote such situations by letters $a_{ijk}$ where $i,j,k$ are numbers of points (this triple of numbers is unordered).

When considering four collinear points, we see that {\em the tetrahedron~(Za\-mo\-lod\-chi\-kov, {\rm see, for example, \cite{etin}}) equation} emerges. Namely, having a dynamics with a quadruple point and slightly perturbing it, we get a dynamics, where this quadruple point splits into four triple points.

Writing it algebraically, we get:

$$a_{ijk}a_{ijl}a_{ikl}a_{jkl}=a_{jkl}a_{ikl}a_{ijl}a_{ijk}.$$

\begin{definition}
The groups $G_{n}^{k}$ are defined as follows.
$$G_{n}^{k} = \langle a_{m} | (1),(2),(3) \rangle,$$
where the generators $a_{m}$ are indexed by all $k$-element subsets of $\{1,\cdots, n\}$, the relation (1) means
\begin{center}
$(a_{m})^{2}=1$ for any unordered sets $m \subset \{1,\cdots, n\}, Card(m)=k$;
\end{center}
(2) means
\begin{center}
$a_{m}a_{m'} = a_{m'}a_{m},$ if $Card(m\cap m') < k-1$;
\end{center}
and, finally, the relation (3) looks as follows. For every set $U \subset \{1,\cdots, n\}$ of cardinality $(k+1)$, let us order all its k-element subsets arbitrarily and denote them by $m^{1}, \cdots, m^{k+1}$. Then (3) is:

$$a_{m^{1}}\cdots  a_{m^{k+1}} = a_{m^{k+1}}\cdots  a_{m^{1}}.$$
\end{definition}

This situation with the Zamolodchikov equation happens almost everywhere, hence, I formulated the following principle: \\

{\em if dynamical systems describing the motion of $n$ particles possess a nice codimension one property governed by exactly $k$ particles, then these dynamical systems admit a topological invariant valued in $G_{n}^{k}$}. \\

In topological language, it means that we get a certain homomorphism from some fundamental group of a configuration space to the groups $G_{n}^{k}$.

Collecting all results about the $G_{n}^{k}$ groups, I taught a half-year course of lectures in the Moscow State University entitled ``Invariants and Pictures'' and a 2-week course in Guangzhou. The notes taken by my colleagues I.\,M.~Nikonov\footnote{I.M.~Nikonov coauthored my first published paper about $G_{n}^{k}$.}, D.\,A.~Fedoseev and S.~Kim were the starting point for the present survey.


Since that time, my seminar in Moscow, my students and colleagues in Moscow, Novosibirsk, Beijing, Guangzhou, and Singapore started to study the groups $G_{n}^{k}$, mostly from two points of view:

{\bf From the topological point of view,} which spaces can we study?

Besides the homomorphisms from the pure braid group $PB_{n}$ to $G_{n}^{3}$ and $G_{n}^{4}$, I just mention that I invented braids for higher-dimensional spaces (or projective spaces).

Of course, the configuration space $C(\R^{k-1},n)$ is simply connected for $k>3$ but if we take some {\em restricted} configuration space $C'(\R^{k-1},n)$, it will not be simply connected any more and will lead to a meaningful notion of higher dimensional braid.

What sort of the restriction do we impose? On the plane, we consider just braids, so we say that no two points coincide. In $\R^{3}$ we forbid collinear triples, in $\R^{4}$ we forbid coplanar quadruple of points.

When I showed the spaces I study to my coauthor, Jie Wu, he said: look, these are $k$-regular embeddings, they go back to Carol Borsuk. Indeed, after looking at some papers by Borsuk, I saw similar ideas were due to P.\,L.~Chebysheff (\cite{Borsuk, Chevyshev_poly}).

By the way, once Wu looked at the group $G_{n}^{k}$, he immediately asked about the existence of simplicial group structure on such groups,  the joint project we are working on now with S. Kim, J. Wu Jie, F. Li.

An interested reader may ask whether such braids exist not only for $\R^{k}$ (or $\R{}P^{k}$), but also for other manifolds, the question we shall touch on later.


{\bf From the algebraic point of view,} why are these groups good, how are they related to other groups, how to solve the word and the conjugacy problems, etc.?

It is impossible to describe all directions of the $G_{n}^{k}$ group theory in the survey, I just mention some of them.

For properties of $G_{n}^{k}$, we can think of them as $n$-strand braids with $k$-fold strand intersection.

Like ${n\choose k}={{n-1}\choose k}+{{n-1}\choose {k-1}}$, there are nice ``strand forgetting'' and ``strand deletion'' maps to $G_{n-1}^{k}$ and $G_{n-1}^{k-1}$, see Fig.~\ref{(n,k)_(n-1,k)_(n-1,k-1)}.

\begin{figure}[h!]
\begin{center}
 \includegraphics[width = 10cm]{pics/maps_from_gnk.eps}

\end{center}

\caption{Maps from $G_{n}^{k}$ to $G_{n-1}^{k}$ and $G_{n-1}^{k-1}$}\label{(n,k)_(n-1,k)_(n-1,k-1)}
\end{figure}



The groups $G_{n}^{k}$ have lots of epimorphisms onto free products of cyclic groups; hence, invariants constructed from them are powerful enough and easy to compare.

For example, the groups $G_{n}^{2}$ are commensurable with some Coxeter groups of special type, see Fig. \ref{Gn2_Cox_Cay}, which immediately solves the word problem for them.

 \begin{figure}[h]
\begin{center}
 \includegraphics[width = 8cm]{pics/hexagonal_tiling.eps}

\end{center}

\caption{The Cayley graph of the group $G_{3}^{2}$ and the Coxeter group $C(3,2)$}\label{Gn2_Cox_Cay}
\end{figure}

As Diamond lemma works for Coxeter groups, it works for $G_{n}^{2}$, and in many other places.

In general, we may say that the words from $G^k_n$ for $n=k+1$ can be realised as braids on $\RP^{k-1}$ describing dynamics of $k+1$ points, and for the case of $n>k+1$ we should investigate partial flag manifolds. That leads to Grassmanians and resolution of singularities.

After a couple of years of study of $G_{n}^{k}$, I understood that I was not completely free and this approach was still somewhat restrictive. Well, we can study braids, we can invent braids in $\R^{n}$ and $\R{}P^{n}$, but what if we consider just braids on a $2$-surface? What can we study then? The property ``three points belong to the same line'' is not quite good even in the metrical case because even if we have a Riemannian metric on a $2$-surface of genus $g$, there may be infinitely many geodesics passing through two points. Irrational cables may destroy the whole construction.

Then I decided to transform the ``$G_{n}^{k}$-point of view'' to make it more local and more topological. Assume we have a collection of points in a $2$-surface and seek $G_{n}^{4}$-property: four points belong to the same circle.





Consider a $2$-surface of genus $g$ with $N$ points on it.
We choose $N$ to be sufficiently large and put points in a position to
form the centers of Vorono\"{\i} cells. It is always possible for the
sphere $g=0$, and for the plane we may think that all our points live inside
a triangle forming a Vorono\"{\i} tiling of the latter.

We are interested in those moments when the combinatorics of the Vorono\"{\i}
tiling changes, see Fig. \ref{tiling_change}.

\begin{figure}[h]
\begin{center}
 \includegraphics[width = 80mm]{pics/tiling_change.eps}
\end{center}
\caption{Vorono\"{\i} tiling change}\label{tiling_change}
\end{figure}

This corresponds to a flip, the situation when four {\em nearest points belong to the same circle}.
This means that no other point lies inside the circle passing through these four ones.

The most interesting situation of codimension $2$ corresponds to five points belonging
to the same circle.

This leads to the relation:~$$d_{1234}d_{1245}d_{2345}d_{1235}d_{1345}=1.$$

Note that unlike the case of $G_{n}^{4}$, here we have five terms, not ten.
What is the crucial difference? The point is that if we have five points in the neighbourhood
of a circle, then every quadruple of them appears to be on the same circle {\em twice},
but one time the fifth point is outside the circle, and one time it is inside the circle. We denote the set $\{1,\dots, n\}$ by $\bar{n}$ and introduce the following

\begin{definition}
The group $\Gamma_{n}^{4}$ is the group given by group presentation generated by $\{ d_{(ijkl)}~|~ \{i,j,k,l\} \subset \bar{n}, |\{i,j,k,l\}| = 4\}$ subject to the following relations:

\begin{enumerate}
\item $d_{(ijkl)}^{2} = 1$ for $\{ i,j,k,l\} \subset \bar{n}$,
\item $d_{(ijkl)}d_{(stuv)} = d_{(stuv)}d_{(ijkl)}$, for $| \{i,j,k,l\} \cap \{s,t,u,v\} | < 3$,
\item $d_{(ijkl)}d_{(ijlm)}d_{(jklm)}d_{(ijkm)}d_{(iklm)} = 1$ for distinct $i,j,k,l,m$,
\item $d_{(ijkl)}=d_{(kjil)}=d_{(ilkj)}=d_{(klij)}=d_{(jkli)}=d_{(jilk)}=d_{(lkji)}=d_{(lijk)}$, for distinct $i,j,k,l$.
\end{enumerate}
\end{definition}

Just like we formulated the $G_{n}^{k}$ principle, here we could formulate the $\Gamma_{n}^{k}$
principle in whole generality, but we restrict ourselves with several examples.

%First, when we deal with higher dimensional manifolds, in this way we invent {\em braids for arbitrary manifolds of arbitrary dimension}, and these elements turn out to have a {\em nice map to the groups $\Gamma_{n}^{k}$}.

%Even in the case of usual braids on $2$-surfaces, we get interesting maps to $\Gamma_{n}^{4}$.

It turns out that groups $\Gamma_{n}^{4}$ have nice presentation coming from
{\em the Ptolemy relation} and the cluster algebras. The Ptolemy relation
$$xy=ac+bd$$ says that the product of diagonals of an inscribed quadrilateral
equals the sum of products of its opposite faces, see Fig. \ref{flip_ind}.

\begin{figure}[h]
\begin{center}
 \includegraphics[width = 90mm]{pics/flip_ind.eps}
\end{center}
\caption{The Ptolemy relation}\label{flip_ind}
\end{figure}

We can use it when considering
triangulations of a given surface: when performing a flip, we replace one diagonal $(x)$ with the other diagonal $(y)$ by using this relation.
It is known that if we consider all five triangulations of the pentagon and
perform five flips all the way around, we return to the initial triangulation
with the same label.

This well known fact gives rise to presentations of $\Gamma_{n}^{4}$.

Thus, by analysing the groups $\Gamma_{n}^{4}$, we can get

\begin{enumerate}
\item Invariants of braids on $2$-surfaces valued in polytopes;
%\item Invariants of knots;
\item Relations to groups $G_{n}^{4}$;
\item Braids on 3-manifolds.
\end{enumerate}

Going slightly beyond, we can investigate braids in $\R^{3}$ (invented by myself) and the configuration space of polytopes. Indeed, when studying bifurcations of simplicial polytopes in tree-space is similar to studying braids: crucial moments when four points belong to the same facet and the combinatorial structure changes are similar to those moments when four points belong to the same circle with no points inside.

We will not say much in the introduction about the groups $\Gamma_{n}^{k}$ for $k>4$ (we discuss them later, though, see Section \ref{sec:gamma_n_5}).
The main idea is:
\begin{enumerate}
\item Generators (codimension 1) correspond to simplicial $(k-2)$-polytopes $k$ vertices;
\item The most interesting relations (codimension 2) correspond to $(k-2)$-polytopes with $k+1$ vertices.
\item Roughly speaking, the most interesting relation in these groups deals with ``higher associativity''.
\end{enumerate}

It would be extremely interesting to establish the connection between $G_{n}^{k}$ with the Manin--Schechtmann ``{\em higher braid groups}'' \cite{ManinSchechtmann} where the authors study the fundamental group of complements to some configurations of {\em complex hyperplanes}.

It is also worth mentioning, that the relations in the group $G_n^2$ resemble the relations in {\em Kirillov--Fomin algebras} \cite{KirFom}. For that reason it seems interesting to study the interconnections between those objects.

Finally, our invariants may not be just group-valued: some variations of $G_{n}^{k}$ admit simplicial group structures, which is studied now in a joint work with S. Kim, F. Lee and J. Wu.


The survey culminates with the {\em manifold of triangulations} and invariants of arbitrary manifolds.

The space of triangulations of a manifold with $N$ points has been considered since a long ago. It is known that triangulations are related to each other by Pachner moves.

The structure on the set of triangulations, its relations to associahedra, permutohedra, etc. has been widely studied, see \cite{nab,GelKapZel} and references therein. This structure is related to lots of different areas of mathematics. Say, Stasheff's polytopes were first introduced by Stasheff (following Milnor and Adams) in order to construct H-associativity on topological spaces.

Interestingly, the space of all triangulations of a sphere, the space of all simplicial polytopes of a given dimension and similar objects were considered by many authors in many directions, but, to the best of my knowledge, the ``canonical'' group action on such objects has not been introduced.


In the present survey we introduce {\em the braid group for manifolds of arbitrary dimension.} If the manifold were just $\R^{k-1}$ ($\RP^{k-1}$) we would consider the restricted configuration space by deleting local codimension $2$ set from the set of whole triangulations. We get an (open) manifold, whose fundamental groups can be studied by means of groups $\Gamma_{n}^{k}$.

Depending on the point of view, {\em geometrical} or {\em topological}, we can define different manifolds of triangulations with different braid groups. These groups are naturally mapped to the corresponding $\Gamma_{n}^{k}$. Such spaces, triangulations, flips, cluster algebras were studied in \cite{KirFom} (see also references therein) but the group structure was missing.


Formulating this principle concisely,  we seek nice codimension $2$ property which would create a non-trivial group. Nice codimension $1$ property gives rise to the local condition, which guarantees that these groups have a nice map to $\Gamma_{n}^{k}$; algebraic nature of $\Gamma_{n}^{k}$ allows one to ``take a picture'' of the discriminant set to get various presentations of the groups into algebraic objects (keep in mind the Pachner move).

In summary, we have constructed two families of groups $G_{n}^{k},\Gamma_{n}^{k}$ which are friendly to various well-known objects (braid groups, Coxeter groups, cluster algebras, configuration spaces, spaces of polytopes), touch different theories and areas of study (as diverse as picture-valued invariants and combinatorics of the Diamond lemma), lead to the construction of new invariants of manifolds, to the invention of new objects (braids for higher dimensional spaces), and motivate new areas of research in topology, algebra and geometry. \\

The authors would like to express their heartfelt gratitude to L.\,A~Bokut', H.~Boden, J.\,S.~Carter, A.\,T.~Fomenko, S.\,G.~Gukov, Y.~Han, D.\,P.~Ilyutko, A.\,B.~Karpov, R.\,M.~Kashaev, L.\,H.~Kauffman, M.\,G.~Khovanov, A.\,A.~Klyachko, P.\,S.~Kolesnikov, I\,G.~Korepanov, S.\,V.~Matveev, A.\,Yu.~Olshanskii, W.~Rushworth, G.\,I.~Sharygin, V.\,A.~Vassiliev, Jun Wang, J.~Wu and Zerui~Zhang for their interest and various useful discussions on the present work. We are grateful to Efim~I.~Zelmanov for pointing out the resemblance between the groups $G_{n}^{2}$ and Kirillov-Fomin algebras. \\

The first named author was supported by the Laboratory of Topology and Dynamics, Novosibirsk State University (grant No. 14.Y26.31.0025 of the government of the Russian Federation).  The second named author was supported by the program ``Leading Scientific Schools'' (grant no. NSh-6399.2018.1, Agreement No. 075-02-2018-867) and by the Russian Foundation for Basic Research (grant No. 19-01-00775-a). The fourth named author was supported by the program ``Leading Scientific Schools'' (grant no. NSh-6399.2018.1, Agreement No. 075-02-2018-867) and by the Russian Foundation for Basic Research (grant No. 18-01-00398-a).

==> section_6_old.tex <==
\section{Dynamical systems and their properties}\label{sect:dyn_sys}

Given a topological space $\Sigma$, called the {\em configuration
space}; the elements of $\Sigma$ will be referred to as {\em
particles}. The topology on $\Sigma^{N}$ defines a natural topology
on the space of all continuous mappings $[0,1]\to \Sigma^{N}$; we
shall also study mappings $S^{1}\to \Sigma^{N}$, where
$S^{1}=[0,1]/\{0=1\}$ is the circle; these mappings will naturally
lead to {\em closures} of $k$-braids.

Let us fix positive integers $n$ and $k$.

The   {\em space of admissible dynamical systems} ${\cal D}$ is a
closed subset in the space of all maps $[0,1]\to \Sigma^{n}$.


A {\em dynamical system}\index{Dynamical system} is an element $D$ of $\mathcal D$. By a {\em state} of $\mathcal D$ we mean the ordered set of particles $D(t)\in
\Sigma^{n}$. Herewith, $D(0)$ and $D(1)$ are called {\em the initial
state} and {\em the terminal state}.

As usual, we shall fix the initial state and the terminal state and
consider the set of admissible dynamics with such initial and
terminal states.

We shall also deal with {\em cyclic dynamical system}, where $D(0)=D(1)$.

We say that a property ${\cal P}$ defined for subsets of the set
of $n$ particles from $\Sigma$ is {\em $k$-good}\index{$k$-good property}, if the following
conditions hold:

\begin{enumerate}

\item if this property holds for some set of particles then it holds for every subset of this set;


\item this property holds for every set consisting of $k-1$ particles among $n$ ones (hence, for every smaller set);

\item fix $k+1$ pairwise distinct numbers $i_{1},\dots,i_{k+1}, i_{j}\in\{1,\dots,n\}$;
if the property ${\cal P}$ holds for particles with numbers
 $i_{1},\dots, i_{k}$ and for the set of particles with numbers $i_{2},\dots, i_{k+1}$, then it holds
 for the set of all
$k+1$ particles $i_{1},\dots, i_{k+1}$.


\end{enumerate}

\begin{remark}
Besides {\em statically good properties} ${\cal P}$,
which are defined for subsets of the set of particles regardless the
state of the dynamics, one can talk about {\em dynamically good}
properties, which can be defined for states considered in time.
\end{remark}

%The simplest example is the motion of points in the Euclidian space
%$\R^{N}$. Here for $k$-good property we take the property of points
%to lie on a fixed $(k-2)$-plane ($k\le N$).

\begin{remark}
Our main example deals with the case $k=3$, where for particles we
take different points on the plane $\Sigma = \R^2$, and ${\cal P}$ is the property
of points to belong to the same line. In general, particles may be
more complicated objects than just points.
\end{remark}

Let ${\cal P}$ be a $k$-good property defined on a set of $n$
particles, $n>k$. For each  $t\in [0,1]$ we shall fix the
corresponding state of particles, and pay attention to those $t$ for
which there is a set $k$ particles possessing ${\cal P}$; we shall
refer to these moments as  ${\cal P}$-critical (or just {\em
critical}).

\begin{definition}
We say that a dynamical system $D$ is {\em pleasant}\index{Dynamical system!pleasant}, if the set of its critical moments is finite whereas for each critical moment there exists exactly one $k$-index set for which the condition ${\cal P}$ holds (thus, for larger sets the property ${\cal P}$ does not hold). Such an unordered $k$-tuple of indices will be called a {\em multiindex} of critical moments.
\end{definition}

With a pleasant dynamical system we associate its {\em type}
$\tau(D)$, which will be the set of multiindices $m^{1},\dots,
m^{N}$, written as $t$ increases from $t=0$ to $t=1$.

For each dynamics $D$ and each multiindex $m=(m_{1},\dots, m_{k})$,
let us define the {\em $m$-type} of $D$ as the ordered set $t_{1}<
t_{2}< \dots$ of values of $t$ for which the set of particles
$m_{1},\dots, m_{k}$ possesses the property ${\cal P}$.

Notation: $\tau_{m}(D)$. If the number $l$ of values $t_{1}<\dots<
t_{l}$ is fixed, then the type can be thought of as a point in
$\R^{l}$ with coordinates $t_{1},\dots, t_{l}$.

\begin{definition}
By the {\em type} of a dynamical system, we mean the set of all its
types $\tau_{m}(D)$. Notation: $\tau(D)$.
\end{definition}

If $D$ is pleasant, then these set are pairwise disjoint.

\begin{definition}
Fix a number $k$ and a $k$-good property  ${\cal P}$. We say that  $D$
is  {\em ${\cal P}$-stable}\index{Dynamical system!stable}, if there is a neighbourhood $U(D)$,
where each dynamical system $D'\in U\setminus\{D\}$ is pleasant, whereas for each
multiindex $m$ (consisting of $k$ indices), the number $l$ of
critical values corresponding to this multiindex $U(D)$ is the same, the type
$\tau_{m}$ is a continuous mapping $U(D)\to \R^{l}$.
\end{definition}

We shall often say {\em pleasant dynamical systems} or {\em stable
dynamical systems} without referring to ${\cal P}$ if it is clear
from the context which ${\cal P}$ we mean.


\begin{definition}
A {\em deformation} is a continuous path $s:[0,1]\to {\cal D}$ in
the space of admissible dynamical systems, from a stable pleasant
dynamics $s(0)$ to another pleasant stable dynamical system $s(1)$.
\end{definition}

\begin{definition}
We say that a deformation $s$ is {\em admissible} if:
\begin{enumerate}


\item the set of values $u$, where $s(u)$ is not pleasant or is not stable, is finite,
and for those $u$ where $s(u)$ is not pleasant, $s(u)$ is stable.


\item inside the stability intervals, the $m$-types are
continuous for each multiindex $m$.

\item for each value $u=u_{0}$, where $s(u_{0})$ is not pleasant, exactly one of the two following
cases occurs:


\begin{enumerate}
\item There exists exactly one $t=t_{0}$ and exactly one $(k+1)$-tuple
$m=(m_{1},\dots, m_{k+1})$ satisfying ${\cal P}$ for this $m$
(hence, ${\cal P}$ does not hold for larger sets).

Let ${\tilde m}_{j}=m\setminus \{m_{j}\},j=1,\dots, k+1$  For types
$\tau_{{\tilde m}_{j}}$, choose those coordinates $\zeta_{j}$, which
correspond to the value $t=t_{0}$. It is required that for all these
values  $u_{0}$ all functions $\zeta_{j}(u)$ are smooth, and all
derivatives $\frac{\partial \zeta_{j}}{\partial{u}}$ are pairwise
distinct;


\item there exists exactly one value $t=t_{0}$ and exactly two
multiindices  $m=\{m_{1},\dots, m_{k}\}$ and $m'=\{m'_{1},\dots,
m'_{k}\}$ for which  ${\cal P}$  holds; we require that $Card(m\cap
m')<k-1$.
\end{enumerate}

\item For each value $u$, where the dynamical system $s(u)$ is not
stable, there exists a value $t=t_{0}$, which is not critical for
$D_{u}$, and a multiindex $\mu=(\mu_{1},\dots,\mu_{k})$, for which
the following holds. For some small  $\eps$ all dynamical systems
$D_{u_0}$ for $u_{0}\in (u-\eps,u)$ and $u_{0}\in (u,u+\eps)$ are
stable (for $\delta<\eps$), and the type $\tau_{\mu}(D_{u+\delta})$
differs from the type $\tau_{\mu}(D_{u-\delta})$ by an
addition/removal of two identical multiindices  $\mu$ in positions close to $t_{0}$.



\end{enumerate}
\end{definition}

For the space of deformation $\mathfrak{D}$, one defines an induced topology.


\begin{definition} We say that a $k$-good property ${\cal P}$ is $k$-{\em correct} for the space of admissible dynamical
systems, if the following conditions hold:

\begin{enumerate}

\item In each neighbourhood of any dynamical system $D$ there exists a pleasant dynamical system $D'$.

\item For each deformation $s$ there exists an {\em admissible} deformation with the same ends $s'(0)=s(0),s'(1)=s(1)$.

\end{enumerate}

\end{definition}

\begin{definition}
We say that two dynamical systems $D_{0},D_{1}$ are {\em equivalent}, if there exists a deformation $s, s(0)=D_{0},s(1)=D_{1}$.
\end{definition}

Thus, if we talk about a correct  ${\cal P}$-property, we can talk
about an admissible deformation when defining the equivalence.


\subsection{The group $G_{n}^{k}$}

Let us now pass to the definition of the {\em $n$-strand free
$k$-braid group $G_n^k$}\index{$G_n^k$}\index{Braid!free $k-$}.

Consider the following $n \choose k$ generators
$a_{m}$, where $m$ runs the set of all unordered $k$-tuples
$m_{1},\dots, m_{k},$ whereas each $m_{i}$ are pairwise distinct
numbers from $\left\{1,\dots, n\right\}$.

For each unordered $(k+1)$-tuple $U$ of distinct indices $u_{1},\dots, u_{k+1} \in
\{1,\dots, n\}$, consider the $k+1$ sets $m^{j}=U\setminus
\{u_{j}\}, j=1,\dots, k+1$. With $U$, we associate the relation

\begin{equation}\label{eq:gnk_tetrahedron_relation}
a_{m^1}\cdot a_{m^2}\cdots a_{m^{k+1}}= a_{m^{k+1}}\cdots a_{m^2}\cdot a_{m^1}
\end{equation}
for two tuples $U$ and ${\bar U}$, which differ by order reversal,
we get the same relation.

Thus, we totally have
$\frac{(k+1)! {n \choose k+1}}{2}$ relations.

We shall call them the {\em tetrahedron relations}\index{Tetrahedron relation}. Note that those relations appear in physics, see \cite{etin}.

For $k$-tuples  $m,m'$ with $Card(m\cap m')<k-1$, consider the {\em
far commutativity relation:}\index{Far commutativity}

\begin{equation}\label{eq:gnk_far_commutativity_relation}
a_{m}a_{m'}=a_{m'}a_{m}.
\end{equation}

Note that the far commutativity relation can occur only if $n>k+1$.

In addition, for all multiindices $m$, we write down the following
relation:

\begin{equation}\label{eq:gnk_order2_relation}
a_{m}^{2}=1.
\end{equation}

\begin{definition}\label{def:gnk}
The {\em $k$-free braid group} $G_{n}^{k}$ is defined as the quotient group of the free group generated
by all $a_{m}$ for all multiindices $m$  by relations~\eqref{eq:gnk_tetrahedron_relation}, \eqref{eq:gnk_far_commutativity_relation} and
\eqref{eq:gnk_order2_relation}.
\end{definition}

\begin{example}
The group $G_{3}^{2}$ is $\langle
a,b,c\,|\,a^{2}=b^{2}=c^2=(abc)^{2}=1\rangle,$ where
$a=a_{12},b=a_{13},c=a_{23}$, the symmetric group $S_3$ on three letters $a,b,c$.

Indeed, the relation $(abc)^{2}=1$ is equivalent to the relation
$abc=cba$ because of $a^{2}=b^{2}=c^{2}=1$. This obviously yields
all the other tetrahedron relations.
\end{example}

\begin{example}
The group $G_{4}^{3}$ is isomorphic to $\langle
a,b,c,d\,|\,a^{2}=b^{2}=c^{2}=d^2=1,(abcd)^{2}=1,(acdb)^{2}=1,(adbc)^{2}=1\rangle$.
Here $a=a_{123},b=a_{124},c=a_{134},d=a_{234}.$

It is easy to check that instead of $\frac{4!}{2}=12$ relations, it
suffices to take only $\frac{3!}{2}$ relations.
\end{example}



By the {\em length} of a word we mean the number of letters in
this word, by the {\em complexity of a free $k$-braid} we mean the
minimal length of all words representing it. Such words will be
called {\em minimal representatives}. The tetrahedron relations (in
the case of free $2$-braids we call them the {\em triangle
relations}) and the far commutativity relations do not change the
complexity, and the relation $a_{m}^{2}=1$ increases or decreases
the length by $2$.



As usual in the group theory, it is natural to look for minimal
length words representing the given free $k$-braid.

If we deal with conjugacy classes of free $k$-braids, one deals with
the length of cyclic words.

The number of words of fixed length in a finite alphabet is
finite; $k$-braids and their conjugacy classes are the main
objects of the present paper.

Let us define the following two types of homomorphisms for free
braids. For each $l=1,\dots, n$, there is an  {\em index forgetting
homomorphism}\index{Homomorphism!index forgetting} $f_{l}: G_{n}^{k}\to G_{n-1}^{k-1}$; this homomorphism
takes all generators $a_{m}$ with multiindex $m$ not containing $l$
to the unit element of the group, and takes the other generators
$a_{m}$ to $a_{m'}$, where $m'=m\setminus \{l\}$; this operation is
followed by the index renumbering.

The  {\em strand-deletion homomorphism}\index{Homomorphism!strand-deletion} $d_{j}$ is defined as a
homomorphism  $G_{n}^{k}\to G_{n-1}^{k}$; it takes all generators
$a_{m}$ having multiindex containing $j$ to the unit element; after
that we renumber indices.

The free $2$-braids (called also {\em pure free braids}) were
studied in~ \cite{knot_parity, MW, M3}.

For free $2$-braids, the following theorem holds.

\begin{theorem}\label{theo2}
Let $b'$ be a word representing a free $2$-braid $\beta$. Then every
word $b$ which is a minimal representative of  $\beta$, is
equivalent by the triangle relations and the far commutativity
relation to some subword of the word $b'$.

Every two minimal representatives $b_{1}$ and $b_{2}$ of the same free
$2$-braid  $\beta$ are equivalent by the triangle relations and the
far commutativity relations.
\end{theorem}


Thus, for free $2$-braids, the recognition problem can be solved by
means of considering its minimal representative.

The main idea of the proof of this theorem is similar to the
classification of homotopy classes of curves in $2$-surfaces due to
Hass and Scott~\cite{HS}: in order to find a minimal representative,
one looks for ``bigon reductions''  until possible, and the final
result is unique up to third Reidemeister moves for the exception of
certain special cases (multiple curves etc). For free $2$-braids
``bigon reductions'' refer to some cancellations of generators
similar generators $a_{m}$ and $a_{m}$ in good position with respect
to each other, see Fig.~\ref{bigon}, the third Reidemeister move
correspond to the triangle relations, and the far commutativity does
not change the picture at all~\cite{M3}.

Algebraically, this reduction process stems from the gradient descent algorithm in Coxeter groups.%, see Theorem~\ref{th:gn2_coxeter}.

For us, it is crucial to know that {\em when looking at a free
$2$-braid, one can see which pairs of crossings can be cancelled.}
Once we cancel all possible crossings, we get an invariant picture.

Thus, {\em we get a complete picture-valued invariant of a free
$2$-braid}.

Theorem \ref{theo2} means that this picture (complete invariant)
occurs as a sub-picture in every picture representing the same free
$2$-braid.

However, various homomorphisms  $G_{n}^{k}\to G_{n-1}^{k-1}$, whose
combination lead to homomorphisms of type $G_{n}^{k}\to
G_{n-k+2}^{2}$, allow one to construct lots of invariants of groups
$G_{n}^{k}$ valued in {\em pictures}.

In particular, these pictures allow one to get easy estimates for the
complexity of braids and corresponding dynamics.

%Free $k$-braids will be considered in a separate publication.

\subsection{The Main Theorem on dynamical systems invariants}


Let ${\cal P}$ be a  $k$-correct property on the space of admissible
dynamical systems with fixed initial and final states.

Let  $D$ be a pleasant stable dynamical system decribing the motion
of $n$ particles with respect to ${\cal P}$. Let us enumerate all
critical values $t$ corresponding to all multiindices for $D$, as
$t$ increases from $0$ to $1$. With $D$ we associate an element
$c(D)$ of $G_{n}^{k}$, which is equal to the product of $a_{m}$,
where $m$ are multiindices corresponding to critical values of $D$
as $t$ increases from $0$ to $1$.



\begin{theorem}\label{thm:gnk_main_theorem}
Let $D_{0}$ and $D_{1}$ be two equivalent stable pleasant dynamics
with respect to ${\cal P}$. Then $c(D_{0})=c(D_{1})$ are equal as
elements of $G_{n}^{k}$.
\end{theorem}

\begin{proof}
Let us consider an admissible deformation $D_{s}$ between $D_{0}$
and $D_{1}$. For those intervals of values $s$, where $D_{s}$ is
pleasant and stable, the word representing $c(D_{s})$, does not
change by construction. When passing through those values of $s$,
where $D_{s}$ is not pleasant or is not stable, $c(D(s))$ changes as
follows:

\begin{enumerate}
\item Let $s_{0}$ be the value of the parameter deformation, for
which the property ${\cal P}$ holds for some $(k+1)$-tuple of
indices at some time $t=t_{0}$. Note that $D_{s_0}$ is stable.

Consider the multiindex $m=(m_{1},\dots, m_{k+1})$ for which ${\cal
P}$ holds at $t=t_{0}$ for $s=s_{0}$. Let ${\tilde
m}_{j}=m\setminus m_{j},j=1,\dots, k+1$ For types $\tau_{{\tilde
m}_{j}}$, let us choose those coordinates $\zeta_{j}$, which
correspond to  the intersection $t$ at $s=s_{0}$. As $s$ changes,
these type are continuous functions with respect to $s$.

Then for small $\eps$, for $u=u_{0}+\eps$, the word $c(D_{s})$ will
contain a sequence of letters $a_{{\tilde m}_{j}}$ in a certain
order. For values  $s=s_{0}-\eps$, the word $c(D_{s})$ will contain
the same set of letters in the reverse order. Here we have used the
fact that $D_{s}$ is stable.


\item If for some  $s=s_{0}$ we have a critical value with two different $k$-tuples $m,m'$
possessing ${\cal P}$ and $Card(m\cap m')<k-1$, then the word
$c(D_{s})$ undergoes the relation (2) as $s$ passes through $s_{0}$;
here we also require the stability of $D_{s_0}$.

\item If at some $s=s_{0}$, the deformation $D_{s}$ is unstable, then $c(D_{s})$
changes according to (3) as $s$ passes  through $s_{0}$. Here we use
the fact that the deformation is admissible.

\end{enumerate}
\end{proof}

Let us now pass to our main example, the classical braid group. Here
distinct points on the plane are particles. We can require that
their initial and final positions are uniformly distributed
along the unit circle centered at $0$.

For ${\cal P}$, we take the property to belong to the same line.
This property is, certainly, $3$-good. Every motion of points where
the initial state and the final state are fixed, can be approximated
by a motion where no more than $3$ points belong to the same
straight line at once, and the set of moments where three points
belong to the same line, is finite, moreover, no more than one set
of $3$ points belong to the same line simultaneously. This means
that this dynamical system is pleasant.

Finally, the correctedness of ${\cal P}$ means that if we take two
isotopic braids in general position (in our terminology: two
pleasant dynamical systems connected by a deformation), then by a
small perturbation we can get an admissible deformation for which
the following holds. There are only finitely many values of the
parameter $s$ with four points on the same line or two triples of
points on the same line at the same moment; moreover, for each such
$s$ only one such case occurs exactly for one value of $t$.

In this example, as well as in the sequel, the properties of being
{\em pleasant} and {\em correct} are based on the fact that every
two {\em general position} states can be connected by a curve passing
through states of codimension $1$ (simplest generation) finitely
many times, and every two paths with fixed endpoints, which can be
connected by a deformation, can be connected by a general position
deformation where points of codimensions $1$ and $2$ occur, the
latter happen only finitely many times.

In particular, the most complicated condition saying that the set of
some $(k+1)$ particles satisfies the property ${\cal P}$, the
corresponding derivatives are all distinct, is also a general
position argument. For example, assuming that some $4$ points belong
to the same horizontal line (event of codimension $2$), we may
require there is no coincidence of any further parameters (we avoid
events of codimension $3$).


From the definition of the invariant $c$, one easily gets the
following
\begin{theorem}
Let $D$ be a dynamical system corresponding to a classical braid.
Then the number of horizontal trisecants of the braid $D$ is not
smaller than the complexity of the free $3$-braid $\beta=c(D)$.
\end{theorem}

Analogously, various geometrical properties of dynamical systems can
be analysed by looking at complexities of corresponding groups of
free $k$-braids, if one can define a $k$-correct property for these
dynamics, which lead to invariants valued in free $k$-braids.

Let us now collect some situations where the above methods can be
applied.

\begin{enumerate}

\item An evident invariant of closed pure classical braids is the conjugacy class of the group $G_{n}^{3}$.
To pass from arbitrary braids to pure braids, one can take some
power of the braid in question.



\item Note that the most important partial case for $k=2$ is the classical Reidemeister braid theory.
Indeed, for a set of points on the plane $Oxy$, we can take for
${\cal P}$ the property that the $y$-coordinates of points coincide.
Then, considering a braid as motion of distinct points in the plane
$z=1-t$ as $t$ changes from $0$ to $1$, we get a set of curves in
space whose projection to $Oxz$ will have intersections exactly in
the case when the property ${\cal P}$ holds. The additional
information coming from the $y$ coordinate, leads one to the
classical braid theory.


\item For classical braids, one can construct invariants for  $k=4$ in a way similar to $k=3$.
In this case, we again take ordered sets of $n$ points on the plane,
and the property ${\cal P}$ means that the set of points belongs to
the same circle or straight line; for three distinct points this
property always holds, and the circle/straight line is unique.

\item With practically no changes this theory can be used for the study of
weavings \cite{Weaves}, collections of projective lines in
$\R{}P^{3}$ considered up to isotopy. Here ${\cal P}$ is the
property of a set of points to belong to the same projective line.
The main difficulty here is that the general position deformation
may contain three lines having infinitely many common horizontal
trisecants. Another difficulty occurs when one of our lines becomes
horizontal; this leads to some additional relations to our groups
$G_{n}^{3}$, which are easy to handle.

\item In the case of points on a $2$-sphere we can define ${\cal P}$ to be the property of
points to belong to the same geodesic. This theory works with an
additional restriction which forbids antipodal points. Some
constraints should be imposed in the case of $2$-dimensional
Riemannian manifolds: for the space of all dynamical systems, we
should impose the restrictions which allow one to detect the
geodesic passing through two points in a way such that if two
geodesics chosen for $a,b$ and for $b,c$ coincide, then the same
geodesic should be chosen for $a,c$.

\item We can use this paradigm to study configurations of balls in a space. A dynamic of balls induces a dynamic of their centers, so any $k$-good property assigns a word in some group $G_n^k$ to the dynamic. The difference between dynamics of balls and ones of a set of points is that the centers of balls can not move too close to each other.

\item In the case of $n$ non-intersecting projective $m$-dimensional planes in $\R{}P^{m+2}$
considered up to isotopy, the theory works as well. Here, in order
to define the dynamical system, we take a one-parameter family of
projective hyperplanes in general position, for particles we take
$(m-1)$-dimensional planes which appear as intersections of the
initial planes with the hyperplane.

The properties of being good, correct etc. follow from the fact that
in general position ``particles'' have a unique same secant line (in
a way similar to projective lines, one should allow the projective
planes not to be straight).
%
For $m=1$ one should take $k=3$, in the general case one takes
$k=2m+1$.

%{\bf This theory will be developed in a separate publication.}

\item This theory can be applied to the study of fundamental groups of various discriminant
spaces, if such spaces can be defined by several equalities and
subsets of these equalities can be thought of as property ${\cal P}$.

\item The case of classical knots, unlike classical links, is a bit more
complicated: it can be considered as a dynamical system, where the
number of particles is not constant, but it is rather allowed for
two particles to be born from one point or to be mutually
contracted.

The difficulty here is that knots do not possess a group structure,
thus, we don't have a natural order on the set of particles.
Nevertheless, it is possible to construct a map from classical knots
to {\em free $3$-knots} (or free $4$-knots) and study them in a way
similar to free $3$-braids (free $4$-braids).
\end{enumerate}

\begin{remark}
In the case of sets of points in space of dimension $3$, the
property of some points to belong to a $2$-plane (or
higher-dimensional plane) is not correct. Indeed, if three points
belong to the same line, then whatever fourth point we add to them,
the four points will belong to the same plane, thus we can get
various multiindices of $4$ points corresponding to the same moment.

The ``triviality'' of such theory taken without any additional
constraints has the simple description that the configuration space
of sets of points in $\R^{3}$ has trivial fundamental group.
\end{remark}

\begin{remark}
In some cases we can reduce one $k$-good properties to others. For example, consider the $4$-good properties $\mathcal P_1$: ``points in the plane lie on the same circle (or the same line)'', and $\mathcal P_2$: ``points in the $3$-dimensional space lie on the same $2$-plane''.

Let $f\colon \R^2\to \R^3$ be the inverse stereographic projection:
$$
f(u,v) = \left(\frac{2u}{u^2+v^2+1}, \frac{2v}{u^2+v^2+1}, \frac{u^2+v^2-1}{u^2+v^2+1}\right)
$$

The image of the map $f$ is the unit sphere without a point, and the image of any circle or line is a circle on the sphere, i.e. an intersection of the sphere and a $2$-plane. Thus, a set $X\subset \R^2$ contains four points which lie on the same circle or line, if and only if the set $f(X)=\{f(x)\}_{x\in X}\subset \R^3$ contains four points which lie on the same $2$-plane. In other words, the property $\mathcal P_1$ can be reduced to the property $\mathcal P_2$.

We can summarise the reasonings above in the following statement.

\begin{proposition}\label{prop:Gn4_good_property_reduction}
Let $C_n(\R^2)$ be the configuration space of ordered sets consisting of $n$ distinct points in $\R^2$, and $C_n'(\R^3)$ be the configuration space of ordered sets consisting of $n$ distinct points in $\R^3$ such that there are no three points which lie on the same line. Then the following diagram is commutative
$$
\xymatrix{
  \pi_1(C_n(\R^2)) \ar[rr]^{f_*} \ar[dr]_{c_{\mathcal P_1}}
                &  &    \pi_1(C_n'(\R^3)) \ar[dl]^{c_{\mathcal P_2}}    \\
                & G_n^4                }
$$
where $c_{\mathcal P_i}$ is the homomorphism of Theorem~\ref{thm:gnk_main_theorem} determined by the property $\mathcal P_i$, $i=1,2$.
\end{proposition}

A construction above can be used for reduction of other $k$-good properties to the basic $k$-property ``points lie on the same hyperplane in $\R^{k-1}$''.

\end{remark}

\subsection{Pictures}

The free $k$-braids can be depicted by strands connecting points
$(1,0),\dots, (n,0)$ to points $(1,1),\dots, (n,1)$; every strand
connects $(i,0)$ to $(i,1)$; its projection to the second coordinate
is a homeomorphism. We mark crossings corresponding $a_{i,j,k}$ by a
solid dot where strands $\#i,\#j,\#k$ intersect transversally.

All other crossings on the plane are artefacts of planar drawing;
they do not correspond to any generator of the group, and they are
encircled, see Fig. \ref{3braid}.

%\begin{figure}
%\centering\includegraphics[width=120pt]{pics/threebr.eps} \caption{The $3$-braid
%$a_{234}a_{123}$} \label{3braid}
%\end{figure}

\begin{figure}[h!]
\begin{minipage}{.4\textwidth}
\begin{center}
 \includegraphics[width =.75\textwidth]{pics/threebr.eps}
\end{center}
%\vspace{-0.4cm}
 \caption{The $3$-braid $a_{234}a_{123}$}\label{3braid}
 \end{minipage}
 \begin{minipage}{.6\textwidth}
 \begin{center}
 \includegraphics[width =.9\textwidth]{pics/red.eps}
 \end{center}
 \caption{The bigon reduction} \label{bigon}
 \end{minipage}
 \end{figure}


The clue for the recognition of free $2$-braids is the {\em bigon
reduction} shown in Fig. \ref{bigon}.

%\begin{figure}[t!]
%\centering\includegraphics[width=240pt]{pics/red.eps} \caption{The bigon
%reduction}\label{bigon}
%\end{figure}

Here we reduce the bigon whose vertices vertices are $X,Y$.

The graph which appears after all possible bigon reductions (with
opposite edge structure at vertices) is a complete invariant of the free $2$-braid (see also~\cite{M3}).
